Adaptive RIS-aided Communications through ML-based Generation of Phase Masks

Reconfigurable Intelligent Surfaces (RISs) are an attractive technology for Millimeter Wave (mmWave) communications due to their ability to passively reflect incident signals. However, current implementations of RIS rely on performing computationally-intensive algorithms offline to generate phase masks, which are stored as a codebook on the embedded microcontroller on the RIS. The codebook size is restricted by the embedded microcontroller's storage capacity, which limits the ability of the RIS to adapt to evolving channel conditions and deployment scenarios. In this demo, we showcase an Machine Learning (ML)-based solution for dynamically generating new phase masks during runtime. Our approach leverages a ML model deployed on the microcontroller for approximating the output of a phase mask generation algorithm, responding to new inputs while remaining smaller than a codebook.

==> acronyms.tex <==
% !TEX root = ../main.tex
%\section*{DeclareAcronymnyms}

% \begin{DeclareAcronymnym}[IMT-Advanced]

\DeclareAcronym{3GPP}{
    short=3GPP,
    long=3rd Generation Partnership Project
}

\DeclareAcronym{ADC}{
    short=ADC,
    long=Analogue-to-Digital Converter
}

\DeclareAcronym{AMPS}{
    short=AMPS,
    long=Advanced Mobile Phone System
}

\DeclareAcronym{AoA}{
    short=AoA,
    long=Angle of Arrival
}

\DeclareAcronym{AoD}{
    short=AoD,
    long=Angle of Departure
}

\DeclareAcronym{AP}{
    short=AP,
    long=Access Point
}
\DeclareAcronym{AR/VR}{
    short=AR/VR,
    long=Augmented/Virtual Reality
}

\DeclareAcronym{ASP}{
    short=ASP,
    long=Antenna Scan Period
}

\DeclareAcronym{BBU}{
    short=BBU,
    long=Baseband Unit
}

\DeclareAcronym{BER}{
    short=BER,
    long=Bit Error Rate
}

\DeclareAcronym{BLER}{
    short=BLER,
    long=Block Error Rate
}

\DeclareAcronym{BS}{
    short=BS,
    long=Base Station
}

\DeclareAcronym{C-MTC}{
    short=C-MTC,
    long=Mission-Critical \acs{MTC}
}

\DeclareAcronym{C-RAN}{
    short=C-RAN,
    % long=Cloud-\ac{RAN}
    long=Centralised-\ac{RAN}
}

\DeclareAcronym{CBRS}{
    short=CBRS,
    long=Citizen's Broadband Radio Service
}

\DeclareAcronym{CCI}{
    short=CCI,
    long=Commonwealth Cyber Initiative
}

\DeclareAcronym{CDM}{
    short=CDM,
    long=Code Division Multiplexing
}

\DeclareAcronym{CDMA}{
    short=CDMA,
    long=Code Division Multiple Access
}

\DeclareAcronym{CDN}{
  short=CDN,
  long=Content Delivery Network
}

\DeclareAcronym{CN}{
    short=CN,
    long=Core Network
}

\DeclareAcronym{CNaaS}{
    short=CNaaS,
    long=\ac{CN} as a Service
}

\DeclareAcronym{CORD}{
    short=CORD,
    long=Central Office Re-architectured as a Datacenter
}

\DeclareAcronym{COTS}{
    short=COTS,
    long=Commercial-Off-The-Shelf
}

\DeclareAcronym{CRUD}{
  short=CRUD,
  long={Create, Read, Update, Delete}
}

\DeclareAcronym{CSMF}{
    short=CSMF,
    long=Communication Service Management Function
}

\DeclareAcronym{CP}{
    short=CP,
    long=Cloud Provider
    %long=Cyclic Prefix
}

\DeclareAcronym{CR}{
    short=CR,
    long=Cognitive Radio
}

\DeclareAcronym{CriC}{
    short=CriC,
    long=Critical Communication
}

\DeclareAcronym{CS}{
    short=CS,
    long=Cyclic Suffix
}

\DeclareAcronym{CSI}{
    short=CSI,
    long=Channel State Information
}

\DeclareAcronym{CSP}{
    short=CSP,
    long={Communication Service Provider}
}

\DeclareAcronym{D-AMPS}{
    short=D-AMPS,
    long=Digital \acs{AMPS}
}

  \DeclareAcronym{D-RAN}{
    short=D-RAN,
    long=Distributed-\ac{RAN}
}

\DeclareAcronym{DAC}{
    short=DAC,
    long=Digital-to-Analogue Converter
}

\DeclareAcronym{DCN}{
    short=DCN,
    long=Data Centre Network
}

\DeclareAcronym{DEQUE}{
    short=DEQUE,
    long=Double-Ended Queue
}

\DeclareAcronym{DNN}{
    short=DNN,
    long=Deep Neural Network}
\DeclareAcronym{DQN}{
    short=DQN,
    long=Deep Q-Network}
\DeclareAcronym{DDQN}{
    short=DDQN,
    long=Double~Deep Q-Network}
\DeclareAcronym{DRL}{
    short=DRL,
    long=Deep Reinforcement Learning}

\DeclareAcronym{DS-CDMA}{
    short=DS-CDMA,
    long=Direct Sequence \acs{CDMA}
}

\DeclareAcronym{DPP}{
    short=DPP,
    long=Determinantal Point Process
}

\DeclareAcronym{LoS}{
    short=LoS,
    long=Line of Sight
}

\DeclareAcronym{DSA}{
    short=DSA,
    long=Dynamic Spectrum Access
}

\DeclareAcronym{DWDM}{
  short=DWDM,
  long=Dense Wavelength Division Multiplexing
}


\DeclareAcronym{RIS}{
  short=RIS,
  long=Reconfigurable Intelligent Surface 
}

\DeclareAcronym{E2E}{
    short=E2E,
    long=End-to-End
}

\DeclareAcronym{ECC}{
    short=ECC,
    long=Electronic Communications Committee
}

\DeclareAcronym{EDGE}{
    short=EDGE,
    long=Enhanced Data rates for \acs{GSM} Evolution
}

\DeclareAcronym{eMBB}{
    short=eMBB,
    long=Enhanced \acl{MBB}
}

\DeclareAcronym{ML}{
    short=ML,
    long=Machine Learning
}

\DeclareAcronym{EPC}{
  short=EPC,
  long=Evolved Packet Core
}

\DeclareAcronym{EV-DO}{
    short=EV-DO,
    long=Evolution-Data Optimised
}

\DeclareAcronym{eV2X}{
    short=V2X,
    long=Enhanced \ac{V2X}
}

\DeclareAcronym{FCC}{
    short=FCC,
    long=Federal Communications Commission
}

\DeclareAcronym{FDM}{
    short=FDM,
    long=Frequency Division Multiplexing
}

\DeclareAcronym{FDMA}{
    short=FDMA,
    long=Frequency Division Multiple Access
}

\DeclareAcronym{FHSS}{
    short=FHSS,
    long=Frequency-hopping spread spectrum
}

\DeclareAcronym{FM}{
    short=FM,
    long=Frequency Modulation
}

\DeclareAcronym{FPGA}{
    short=FPGA,
    long=Field-Programmable Gate Array
}

\DeclareAcronym{FS}{
    short=FS,
    long=Flow Space
}

\DeclareAcronym{FSK}{
    short=FSK,
    long=Frequency-Shift Keying
}

\DeclareAcronym{GAA}{
    short=GAA,
    long=General Authorized Access
}

\DeclareAcronym{GPIO}{
    short=GPIO,
    long=General Purpose Input/Output
}

\DeclareAcronym{GPP}{
    short=GPP,
    long=general purpose process
}

\DeclareAcronym{GPRS}{
    short=GPRS,
    long=General packet radio service
}

\DeclareAcronym{GRC}{
    short=GRC,
    long=Global Radio Coordinator
}

\DeclareAcronym{GSM}{
    short=GSM,
    long=Global System for Mobile communication
}

\DeclareAcronym{H2H}{
    short=H2H,
    long=Human-to-Human
}

\DeclareAcronym{HetNet}{
    short=HetNet,
    long=Heterogeneous Network
}

\DeclareAcronym{HSDPA}{
    short=HSDPA,
    long=High Speed Downlink Packet Access
}

\DeclareAcronym{HSPA}{
    short=HSPA,
    long=High Speed Packet Access
}

\DeclareAcronym{HSUPA}{
    short=HSUPA,
    long=High-Speed Uplink Packet Access
}

\DeclareAcronym{IA}{
    short=IA,
    long=Initial Access
}

\DeclareAcronym{iDEN}{
    short=iDEN,
    long=Integrated Digital Enhanced Network
}

\DeclareAcronym{IF}{
    short=IF,
    long=Intermediate Frequency
}

\DeclareAcronym{IMT}{
    short=IMT,
    long=International Mobile Telecommunication
}

\DeclareAcronym{IMT-2000}{
    short=IMT-2000,
    long=\aclp{IMT}-2000
}

\DeclareAcronym{IMT-Advanced}{
    short=IMT-Advanced,
    long=\aclp{IMT}-Advanced
}

\DeclareAcronym{INR}{
    short=INR,
    long=Interference-to-Noise Ratio
}

\DeclareAcronym{I/O}{
    short=I/O,
    long=Input/Output
}

\DeclareAcronym{InP}{
    short=InP,
    long=Infrastructure Provider
}

\DeclareAcronym{IoT}{
    short=IoT,
    long=Internet of Things
}

\DeclareAcronym{IPM}{
    short=IPM,
    long=Intra-Pulse Modulation
}

\DeclareAcronym{ISM}{
    short=ISM,
    long={Industrial, Scientific and Medical}
}

\DeclareAcronym{ISP}{
    short=ISP,
    long={Internet Service Provider}
}

\DeclareAcronym{ITU}{
    short=ITU,
    long=International Telecommunication Union
}

\DeclareAcronym{KPI}{
    short=KPI,
    long=Key Performance Indicator
}

\DeclareAcronym{LFM}{
    short=LFM,
    long=Linear Frequency Modulation
}

\DeclareAcronym{LOS}{
    short=LOS,
    long=Line-of-Sight
}

\DeclareAcronym{LRC}{
    short=LRC,
    long=Local Radio Controller
}

\DeclareAcronym{LTE-A}{
    short=LTE-A,
    long=\acs{LTE}-Advanced
}

\DeclareAcronym{LTE-U}{
    short=LTE-U,
    long=\acs{LTE} in unlicensed spectrum
}

\DeclareAcronym{LTE}{
    short=LTE,
    long=Long-Term Evolution
}

\DeclareAcronym{LWA}{
    short=LWA,
    long=\acs{LTE}-\acs{WLAN} aggregation
}

\DeclareAcronym{LXC}{
    short=LXC,
    long=Linux Containers,
    long-plural-form=Linux Containers
}

\DeclareAcronym{M2U}{
    short=M2U,
    long=MHU to USRP
}

\DeclareAcronym{M-MTC}{
    short=MTC,
    long=Massive \acs{MTC}
}

\DeclareAcronym{MBB}{
    short=MBB,
    long=Mobile Broadband
}

\DeclareAcronym{MDP}{
    short=MDP,
    long=Markov Decision Process
}

\DeclareAcronym{MHU}{
    short=MHU,
    long=Mast Head Unit
}

\DeclareAcronym{mmWave}{
    short=mmWave,
    long=Millimeter Wave
}

\DeclareAcronym{MMSE}{
    short=MMSE,
    long=Minimum \acl{MSE}
}

\DeclareAcronym{MANO}{
    short=MANO,
    long=Management and Orchestration
}

\DeclareAcronym{MOCN}{
    short=MOCN,
    long=Multi-Operator \ac{CN}
}

\DeclareAcronym{MORAN}{
    short=MORAN,
    long=Multi-Operator \ac{RAN}
}

\DeclareAcronym{MNO}{
    short=MNO,
    long=Mobile Network Operator
}

\DeclareAcronym{MSE}{
    short=MSE,
    long=Mean Square Error
}

\DeclareAcronym{MTC}{
    short=MTC,
    long=Machine Type Communication
}

\DeclareAcronym{MVNO}{
    short=MVNO,
    long=Mobile Virtual Network Operator
}

\DeclareAcronym{NextG}{
    short=NextG,
    long=Next Generation Mobile Networks
}

\DeclareAcronym{NFV}{
    short=NFV,
    long=Network Function Virtualisation
}

\DeclareAcronym{NIC}{
    short=NIC,
    long=Network Interface Card
}

\DeclareAcronym{NLOS}{
    short=NLOS,
    long=Non-Line-of-Sight
}

\DeclareAcronym{NP}{
    short=NP,
    long=Network Provider
}

\DeclareAcronym{NSMF}{
    short=NSMF,
    long=Network Slice Management Function
}

\DeclareAcronym{NSSMF}{
    short=NSSMF,
    long=Network Slice Subnet Management Function
}

\DeclareAcronym{NMT}{
    short=NMT,
    long=Nordic Mobile Telephone
}

\DeclareAcronym{NS}{
    short=NS,
    long=Network Slice
}

\DeclareAcronym{NSaaS}{
    short=NSaaS,
    long=\ac{NS} as a Service
}

\DeclareAcronym{OCXO}{
    short=OCXO,
    long=Oven-controlled Crystal Oscillator
}

\DeclareAcronym{OFDM}{
    short=OFDM,
    long=Orthogonal Frequency Division Multiplexing
}

\DeclareAcronym{OFDMA}{
    short=OFDMA,
    long=Orthogonal Frequency Division Multiple Access
}

\DeclareAcronym{ONF}{
    short=ONF,
    long=Open Network Foundation
}

\DeclareAcronym{ONOS}{
    short=ONOS,
    long=Open Network Operating System
}

\DeclareAcronym{OOT}{
    short=OOT,
    long=Out-of-Tree
}

\DeclareAcronym{ORCA}{
    short=ORCA,
    long=Orchestration and Reconfiguration Control Architecture
}

\DeclareAcronym{OS}{
    short=OS,
    long=Operational System
}

\DeclareAcronym{OTA}{
    short=OTA,
    long=over-the-air
}

\DeclareAcronym{OTT}{
    short=OTT,
    long=Over-The-Top
}

\DeclareAcronym{PA}{
    short=PA,
    long=Priority Access
}

\DeclareAcronym{PAL}{
    short=PAL,
    long=\ac{PA} License
}

\DeclareAcronym{PBCH}{
    short=PBCH,
    long=Physical Broadcast CHannel
}

\DeclareAcronym{PDC}{
    short=PDC,
    long=Personal Digital Cellular
}

\DeclareAcronym{PER}{
    short=PER,
    long=Packet Error Rate
}

\DeclareAcronym{PHP}{
    short=PHP,
    long=Poisson Hole Process
}

\DeclareAcronym{PLC}{
    short=PLC,
    long=Process Logic Controller
}

\DeclareAcronym{PNF}{
  short=PNF,
  long=Physical Network Function
}

\DeclareAcronym{POCSAG}{
    short=POCSAG,
    long=Post Office Code Standardization Advisory Group
}

\DeclareAcronym{PPP}{
    short=PPP,
    long=Poisson Point Process
}

\DeclareAcronym{PRB}{
    short=PRB,
    long=Physical Resource Block
}

\DeclareAcronym{PRI}{
    short=PRI,
    long=Pulse Repetition Interval
}

\DeclareAcronym{PSD}{
    short=PSD,
    long=Power Spectral Density
}

\DeclareAcronym{PSK}{
    short=PSK,
    long=Phase-Shift Keying
}

\DeclareAcronym{PSS}{
    short=PSS,
    long=Primary Synchronization Signal
}

\DeclareAcronym{PTSN}{
    short=PTSN,
    long=Public Switched Telephone Network
}

\DeclareAcronym{PW}{
    short=PW,
    long=Pulse Width
}

\DeclareAcronym{QoE}{
    short=QoE,
    long=Quality of Experience
}

\DeclareAcronym{QoS}{
    short=QoS,
    long=Quality of Service
}

\DeclareAcronym{RAN}{
    short=RAN,
    long=Radio Access Network
}

\DeclareAcronym{RANaaS}{
    short=RANaaS,
    long=\ac{RAN} as a Service
}

\DeclareAcronym{RAT}{
    short=RAT,
    long=Radio Access Technology,
    long-plural-form=Radio Access Technologies
}

\DeclareAcronym{RF}{
    short=RF,
    long=Radio Frequency
}

\DeclareAcronym{RIC}{
    short = RIC,
    long  = \acs{RAN} Intelligent Controller,
}

\DeclareAcronym{RL}{
    short=RL,
    long=Reinforcement Learning
}

\DeclareAcronym{RRH}{
    short=RRH,
    long=Remote Radio Head
}

\DeclareAcronym{MLP}{
    short=MLP,
    long=Multilayer Perceptron
}
 
\DeclareAcronym{RSRP}{
    short=RSRP,
    long=Reference Signal Received Power
}

\DeclareAcronym{RSRQ}{
    short=RSRQ,
    long=Reference Signal Received Quality
}

\DeclareAcronym{RSS}{
    short=RSS,
    long=Received Signal Strength
}

\DeclareAcronym{RSSI}{
    short=RSSI,
    long=Received Signal Strength Indicator
}

\DeclareAcronym{S/A}{
    short=S/A,
    long=Sensors/Actuators
}

\DeclareAcronym{SAS}{
    short=SAS,
    long=Spectrum Access System
}


\DeclareAcronym{SDH}{
    short=SDH,
    long=Software-Defined Hardware
}

\DeclareAcronym{SDK}{
    short=SDK,
    long=Software Development Kit
}

\DeclareAcronym{SDN}{
    short=SDN,
    long=Software-Defined Network
}

\DeclareAcronym{SDR}{
    short=SDR,
    long=Software-Defined Radio
}

\DeclareAcronym{SDS}{
    short=SDS,
    long=Software-defined Switch,
    long-plural-form=Software-defined Switches
}

\DeclareAcronym{SER}{
    short=SER,
    long=Symbol Error Rate
}

\DeclareAcronym{SFC}{
    short=SFC,
    long=Service Function Chain
}

\DeclareAcronym{SFI}{
    short=SFI,
    long=Science Foundation Ireland
}

\DeclareAcronym{SIR}{
    short=SIR,
    long=Signal-to-Interference Ratio
}

\DeclareAcronym{SINR}{
    short=SINR,
    long=Signal-to-Interference-plus-Noise Ratio
}

\DeclareAcronym{SLA}{
    short=SLA,
    long=Service Level Agreement
}

\DeclareAcronym{SNR}{
    short=SNR,
    long=Signal-to-Noise Ratio
}

\DeclareAcronym{SON}{
    short=SON,
    long=Self Organising Network
}

\DeclareAcronym{SP}{
    short=SP,
    long=Service Provider
}

\DeclareAcronym{SSID}{
    short=SSID,
    long=Service Set Identifier
}

\DeclareAcronym{STAMINA}{
    short=STAMINA,
    long=SofTwAre-defined Mmwave INitial Access
}

\DeclareAcronym{SSS}{
    short=SSS,
    long=Secondary Synchronization Signal
}

\DeclareAcronym{SU}{
    short=SU,
    long=Secondary User
}

\DeclareAcronym{SVL}{
    short=SVL,
    long=Spectrum Virtualization Layer
}

\DeclareAcronym{SSB}{
    short=SSB,
    long= Synchronization Signal Block
}

\DeclareAcronym{TACS}{
    short=TACS,
    long=Total Access Communications System
}

\DeclareAcronym{TDM}{
    short=TDM,
    long=Time Division Multiplexing
}

\DeclareAcronym{TDMA}{
    short=TDMA,
    long=Time Division Multiple Access
}

\DeclareAcronym{THz}{
    short=THz,
    long=Terahertz
}

\DeclareAcronym{TN}{
    short=TN,
    long=Transport Network
}

\DeclareAcronym{TVWS}{
    short=TWS,
    long=TV White Space
}

\DeclareAcronym{UAV}{
    short=UAV,
    long=Unmanned Aerial Vehicle
}

\DeclareAcronym{UE}{
    short=UE,
    long=User Equipment
}

\DeclareAcronym{UHD}{
    short=UHD,
    long=\acs{USRP} Hardware Driver
}

\DeclareAcronym{UMTS}{
    short=UMTS,
    long=Universal Mobile Telecommunications System
}

\DeclareAcronym{URLLC}{
    short=URLLC,
    long=Ultra-Reliable Low Latency Communication
}

\DeclareAcronym{USRP}{
    short=USRP,
    long=Universal Software Radio Peripheral
}

\DeclareAcronym{UUID}{
    short=UUID,
    long=Universally Unique Identifier
}
  \DeclareAcronym{V2X}{
    short=V2X,
    long=Vehicular-to-Everything
}
  \DeclareAcronym{VPN}{
    short=VPN,
    long=Virtual Private Network
}
  \DeclareAcronym{VRB}{
    short=VRB,
    long=Virtual Resource Block
}

\DeclareAcronym{NN}{
  short=NN,
  long=Neural Network
}

\DeclareAcronym{VM}{
  short=VM,
  long=Virtual Machine
}

\DeclareAcronym{VNF}{
  short=VNF,
  long=Virtual Network Function
}

\DeclareAcronym{VRF}{
  short=VRF,
  long=Virtual Radio Function
}

\DeclareAcronym{WCDMA}{
    short=WCDMA,
    long=Wideband Direct Sequence \acs{CDMA}
}

\DeclareAcronym{WiMax}{
    short=WiMax,
    long=Worldwide Interoperability for Microwave Access
}

\DeclareAcronym{WLAN}{
    short=WLAN,
    long=Wireless Local Area Network
}

\DeclareAcronym{WMN}{
    short=WMN,
    long=Wireless Mesh Network
}

\DeclareAcronym{WMWG}{
    short=WMWG,
    long=Wireless and Mobile Working Group
}

\DeclareAcronym{WNV}{
    short=WNV,
    long=Wireless Network Virtualisation
}

\DeclareAcronym{WSN}{
    short=WSN,
    long=Wireless Sensor Network
}

\DeclareAcronym{XaaS}{
    short=XaaS,
    long=Everything as a Service
}

\DeclareAcronym{XVL}{
    short=XVL,
    long=eXtensible Virtualisation Layer
}

\DeclareAcronym{SBM}{
    short=SBM,
    long=Secure Beam Management
}
